Towards Autocomplete Strategies for Visualization Construction

Constructive visualization uses physical data units - tokens - to enable non-experts to create personalized visualizations engagingly. However, its physical nature limits efficiency and scalability. One potential solution to address this issue is autocomplete. By providing automated suggestions while still allowing for manual intervention, autocomplete can expedite visualization construction while maintaining expressivity. We conduct a speculative design study to examine how people would like to interact with a visualization authoring system that supports autocomplete. Our study identifies three types of autocomplete strategies and gains insights for designing future visualization authoring tools with autocomplete functionality. A free copy of this paper and all supplemental materials are available on our online repository https://osf.io/nu4z3/?view_only=594baee54d114a99ab381886fb32a126

==> Discussion_depreciated.tex <==
\section{Discussion}
\label{Sect5}

%\subsection{The Spectrum of Automation}

%\wei{I want to present the same idea about exploring the decision tree(we sketched in Miro), but avoid being complex and introduce more concepts}
%The speculative study helps us identify three autocomplete strategies: Next-step, \textsc{Ghost}, and Mosaic. They represent different degrees of automation assistance in visualization construction. (needs a figure here)\textbf{ Next-step predicts token by token. \textsc{Ghost} shows suggestions chunk by chunk. Mosaic presents a list of final visualization options.} The latter is almost fully automated and commonly used in commercial tools like Excel. 

%\wei{Discuss their advantages/disadvantages, the possibilities of including them in a single tool for different phase(I9)} 

%The tradeoff between exploration(design alternatives) and efforts spend on that. which level of completion, triggers of future work.

%relate the viscomplete things, a huge diversity of autocomplete for visualizations(data level. pipeline, visual marks)

%Limitation: 1, no choices to go back in the decision tree. No correction choices
\subsection{Explore Visualization Decision Tree}
The creation of visualizations through manual assembly requires defining visual mappings token by token.  \begin{wrapfigure}[5]{o}{0.075\textwidth}
    \centering
    \includegraphics[width=0.075\textwidth]{figs/Section5/DecisionTree.jpg}
\end{wrapfigure} This process can be illustrated through a decision tree. Each node represents a token mapping operation. A path from the root to a leaf portrays a mapping schema that defines a visualization. Each autocomplete strategy helps people to explore the decision tree in a different way.

Focusing on sequential steps, one at a time, \textsc{Next-step} provides a preview for child nodes (nodes in pink) of the next level in the decision tree.\begin{wrapfigure}[6]{r}{0.075\textwidth}
    \centering
    \includegraphics[width=0.075\textwidth]{figs/Section5/NextStepTree.jpg}
\end{wrapfigure} The preview demonstrates the possible visual mappings of the token yet to be placed. With the help of the preview, people are able to make a well-informed decision by accepting one node (nodes in red) in the preview at every step. By showing the choices step by step, \textsc{Next-step} helps build a visualization from scratch, especially for non-experts. However, it still requires people to manipulate every token manually, making the authoring process time-consuming. 

\begin{wrapfigure}[6]{r}{0.085\textwidth}
    \centering
    \includegraphics[width=0.085\textwidth]{figs/Section5/GhostTree.jpg}
\end{wrapfigure}The \textsc{Ghost} strategy provides suggestions for paths (marked with ellipses) rather than just individual nodes. By presenting suggestions integrating multiple levels, \textsc{Ghost} allows users to define the visual mapping of multiple tokens at once, making it more efficient than \textsc{Next-step}. As a result, \textsc{Ghost} can speed up the construction process when a desired suggestion is presented. However, to make the most of this strategy, people may need to have some expertise and invest some effort to instruct the system to produce the right suggestion.

\begin{wrapfigure}[5]{r}{0.075\textwidth}
    \centering
    \includegraphics[width=0.075\textwidth]{figs/Section5/MosaicTree.jpg}
\end{wrapfigure} Finally, \textsc{Mosaic} is the ultimate version of \textsc{Ghost}, as it provides suggestions for a selection of complete paths from the root to the leaf nodes. With this high level of automation, \textsc{Mosaic} autocompletes all visual mapping steps required for a visualization, creating a fast and hands-off experience. However, while \textsc{Mosaic} is efficient, it also limits the design alternatives that manual assembly can support, and may compromise the expressive nature of the process. 

\subsection{Automation and Expressivity}
The three autocomplete strategies differ in their degree of automation. \textsc{Next-step} requires manual input for each token, while \textsc{Mosaic} is highly automated and can exclude human participation in the construction process. \textsc{Ghost} falls in between, incorporating both manual assembly and automation. In exploring design options, \textsc{Next-step} provides the most expressivity, while \textsc{Ghost} and \textsc{Mosaic} have a more limited set of available choices. This trade-off suggests that increasing automation can decrease expressivity. Achieving the right balance between automation and expressivity is a complex task that requires careful consideration.

One approach is integrating multiple strategies into a single authoring tool that allows people to switch between them during different phases of visualization creation (I9 exemplifies this idea). For instance, when people want to play with data and explore all possibilities, \textsc{Next-step} can serve as a `non-invasive' assistant. While people have a clear understanding of data and require advanced support, \textsc{Ghost} and \textsc{Mosaic} are valuable tools to expedite the building process and output a desired visualization quickly. Combining these strategies in a single tool can provide users with a flexible and comprehensive toolkit for creating visualizations that balances both automation and expressivity.

%The three autocomplete strategies we discovered differ in the level of automation. \textsc{Next-step} involves manual input for each token, while \textsc{Mosaic} is highly automated and can exclude human participation in the construction process. \textsc{Ghost} falls between the two, incorporating both a degree of manual assembly and automation. At the same time, the design options they afford vary in an opposite direction. \textsc{Next-step} provides the most expressivity while \textsc{Ghost} and \textsc{Mosaic} have limitation of the available choices. It turns out that as automation increases, the expressivity decreases. Therefore, achieving the right balance between automation and expressivity is a complex task that requires careful consideration. %Balancing automation and expressivity is a nuanced task. 

%A potential way is to combine the different strategies during different phases of visualization creation. I9 suggests a potential approach for this problem% in a visualization authoring tool. The first approach is to use a compromised strategy, such as \textsc{Ghost}, which was the most popular strategy among participants (5/11). A well-designed \textsc{Ghost} scheme could provide users with a suitable number of design alternatives without increasing the effort required for exploration.
%: to apply different strategies during different phases of visualization creation. Users often prefer high-level guidance and enough exploration during the early stages for trying out various visualizations, and require greater automation when they know what they want. I9 embodies this idea in their sketches, where users can start by choosing a chart type from a list of visualization templates (\textsc{Mosaic}), build the visualization token by token with autocomplete suggestions (\textsc{Next-step}), and then accelerate the process when enough tokens are placed for the system to provide \textsc{Ghost} predictions.

However, this approach requires further research to address design details, such as the most effective method to switch between strategies, how to assist users in determining when to adopt a particular strategy, and what technology would best support these strategies. Future work could focus on answering these questions to examine the approach further. 


% Our work explores how to utilize autocomplete to automate constructive visualization while keeping expressivity. As a mechanism that aims to help people get desired information quickly, autocomplete is useful for visualization creation, in a general scope. As a semi-automation philosophy, autocomplete fills the gap between fully automated visualization building and fully manual-crafted physicalization. 

% There is a huge space to employ autocomplete for diverse visualization authoring tasks. VisComplete\cite{koop2008viscomplete} adopts it for automating suggestions for visualization pipelines. We explore the techniques of using it for token-based visualization construction. But there are various other ways to use visualization autocomplete, such as data mapping, visual marks.

% \sam{How these strategy relate to exploration of the decision three ? }

% \yvonne{The pruning of the discussion tree could be a nice way to discuss the reults and contrast the strategies. It's not in the paper anymore?} \wei{yeah, currently it is. Do you think it's okay that we didn't mention it before bringing it up in the discussion?}
% \yvonne{I really liked the concept and I think it's an interesting way to think about it. It could even be one the main reasons later for people to cite our paper...}

% \yvonne{Including it only in the discussion could work. I worry a bit though about illustrating it. We're short on space and cannot include another figure.}
% \wei{That's another reason I didn't include it. I can try to describe it verbally, to see if it works}
% \yvonne{COuld it be possible to create small icon figures that could be integrated in the text? Like reduing the tree to the main thing to communicate.}
% \wei{Ahhh, that's a good idea. I love the idea. I am going to do that. THX}
% \yvonne{Great! I need to go now. I'll check back in later this weekend.}

% \sam{How that might be useful for authoring phyicalization tool, fabrication, visualization tool beyond constructive vis ?}
 
\subsection{Limitations}

In our study, we used the search engine metaphor to introduce participants to the concept of autocomplete. While this approach helped participants quickly understand the idea, it also introduced a bias that may have influenced our results. Specifically, some participants focused on text-like autocomplete instead of token-based visualizations, potentially limiting the range of design ideas generated. Additionally, our study did not explore possible iterations of autocomplete or functions to correct or delete tokens that were already placed. As a result, no such features were represented in participants' sketches. %However, since we are interested in high-level design instead of technical details, we do not believe this is to be an issue for this work.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January 2022

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

